Public Bayesian Persuasion: Being Almost Optimal and Almost Persuasive

Persuasion studies how an informed principal may influence the behavior of agents by the strategic provision of payoff-relevant information. We focus on the fundamental multi-receiver model by Arieli and Babichenko (2019), in which there are no inter-agent externalities. Unlike prior works on this problem, we study the public persuasion problem in the general setting with: (i) arbitrary state spaces; (ii) arbitrary action spaces; (iii) arbitrary sender's utility functions. We fully characterize the computational complexity of computing a bi-criteria approximation of an optimal public signaling scheme. In particular, we show, in a voting setting of independent interest, that solving this problem requires at least a quasi-polynomial number of steps even in settings with a binary action space, assuming the Exponential Time Hypothesis. In doing so, we prove that a relaxed version of the Maximum Feasible Subsystem of Linear Inequalities problem requires at least quasi-polynomial time to be solved. Finally, we close the gap by providing a quasi-polynomial time bi-criteria approximation algorithm for arbitrary public persuasion problems that, in specific settings, yields a QPTAS.

==> main.tex <==
\section{The Main Results}

\todoac{restatable}

\begin{restatable*}{theorem}{mainHardness}\label{th:main_hardness}
	Given a $k$-voting instance and assuming ETH, there exists a constant $\epsilon^\ast$ such that, for any $\epsilon\leq\epsilon^\ast$, finding an $(\alpha,\epsilon)$-persuasive signaling scheme requires time $n^{\tilde\Omega(\log n)}$ for any multiplicative or additive factor $\alpha$.
\end{restatable*}

\begin{restatable*}[Bi-criteria QPTAS]{theorem}{qptas}\label{th:qptas}
	Assume $f$ is $\alpha$-approximate, there exists a $\textnormal{poly}\left(d^{\frac{\log(n_r\nAct/\delta)}{\epsilon^2}}\right)$ algorithm that outputs an $\alpha(1-\delta)$-approximate $\epsilon$-persuasive public signaling scheme.
\end{restatable*}

==> related.tex <==
\section{Additional Related Works}

The classic model of Bayesian persuasion is due to \citet{kamenica2011bayesian}. \citet{dughmi2016algorithmic} analyze for the first time Bayesian persuasion from a  computational perspective, focusing on the single receiver case.
Most of the works focus on games with multiple receivers and two basic signaling models: private persuasion, in which the sender has private communication channels, and public persuasion, in which the sender has a single information channel.
In the first setting, \citet{arieli2019private} introduce the model of persuasion with no externalities among the receivers. \citet{arieli2019private} study the setting with binary actions and state spaces, providing a characterization of the optimal signaling scheme in the case of supermodular, anonymous submodular, or supermajority.
\citet{babichenko2016computational} provide a tight $1-1/e$ approximate signaling scheme for monotone submodular sender's utility and show that an optimal private scheme for anonymous utility functions can be found efficiently.
\citet{dughmi2017algorithmic} generalize the previous model to the case of many states of nature.
%
Some works study also public persuasion, showing that designing public signaling scheme is harder.
\citet{bhaskar2016hardness} and \citet{rubinstein2015honest} study public signaling in which two receivers play a zero sum game. In particular, \citet{bhaskar2016hardness} rule out an additive PTAS assuming the planted clique conjecture. \citet{rubinstein2015honest} prove that, assuming the exponential time hypothesis, computing an $\epsilon$-optimal signaling scheme requires quasipolynomial time ($n^{\tilde{\Omega}({log\ n})}$). This result is thight due to an quasipolynomial approximation scheme of \citet{cheng2015mixture}.
Other works study public signaling in games with no externalities. \citet{dughmi2017algorithmic} prove that, even restricting to receivers with binary actions, it's \NPHard\ to obtain a PTAS even for linear objectives. For this reason, most of the work focus on the computation of bicriteria approximation in which the incentive constraints can be violated by a small amount. \citet{cheng2015mixture} design bicriteria approximation for voting setting.
\citet{xu2019tractability} studies public persuasion with binary action spaces and describe a PTAS with a bi-criteria guarantee for monotone submodular sender function. Moreover, under a non-degenerate assumption, \citet{xu2019tractability} provides an algorithm to compute an optimal signaling scheme when the number of states of nature is fixed.
 

